Harnessing Sparsity over the Continuum: Atomic Norm Minimization for Super Resolution

Convex optimization recently emerges as a compelling framework for performing super resolution, garnering significant attention from multiple communities spanning signal processing, applied mathematics, and optimization. This article offers a friendly exposition to atomic norm minimization as a canonical convex approach to solve super resolution problems. The mathematical foundations and performances guarantees of this approach are presented, and its application in super resolution image reconstruction for single-molecule fluorescence microscopy are highlighted.

==> general_model.tex <==
\section{Faster Algorithms}

While the SDP formulation is tractable, its computational complexity is prohibitive when solving large-dimension problems. Fortunately, it is possible to develop tailored algorithms that are significantly faster. For conciseness, we will discuss two approaches based on the Alternating Direction Method of Multipliers (ADMM) \cite{bhaskar2013atomic} and the Alternating Descent Conditional Gradient (ADCG) method \cite{boyd2017alternating}. 
 
\subsection{ADCG}
The ADCG method \cite{boyd2017alternating} is an acceleration of the conditional gradient method, also known as Frank-Wolfe, to solve sparse inverse problems over continuous dictionaries with general convex loss functions. Taking the constrained form of atomic norm denoising as an example, ADCG aims to solve the following problem:
\begin{align*}
    \min_{\bx} \quad & \frac{1}{2} \left\|  \bx - \bz \right\|_2^2 \quad \mbox{subject to} \quad \anorm{\bx} \leq \eta,
\end{align*}
where $\eta>0$ is a regularization parameter. Given an atomic set $\cA_{\mathsf{1D}}$, it directly estimates the support and corresponding coefficients $(\mathcal{T}, \bm{c})$. 

The detailed procedure of ADCG is given in Alg.~\ref{alg:ADCG}. In the $j$th iteration, denote $\mathcal{A}(\mathcal{T}_j)$ as the matrix whose columns are the atoms $\bm{a}(\tau)$ with $ \tau\in \mathcal{T}_j $. ADCG starts by adding a spike to the estimated support $\mathcal{T}_j$ that maximally correlates with the residual of the current estimate, $\mathcal{A}(\mathcal{T}_j)\bm{c}_j - \bm{z}$. Then ADCG iterates between coefficients update via $\ell_1$ minimization, support pruning, and local refinement of the support. The last step leverages the fact that $\bm{a}(\tau)$ is differentiable with respect to $\tau$, and a simple local search via gradient descent allows one to adjust the support to further reduce the loss function. The main computational benefits of ADCG are the absence of semidefinite constraints and small memory footprints, making it highly suitable for large-scale implementations. 

\begin{algorithm}[t]
	\caption{ADCG for atomic norm denoising \cite{boyd2017alternating}}
	\label{alg:ADCG}
	\begin{algorithmic}[H]
		\REQUIRE Observation $\bz$; Parameter $\eta>0$; \\
		\STATE Initialize $\mathcal{T}_0$ to an empty set, $\bm{c}_{0}$ to $\bm{0}$, and $j=0$; \\
		 \textbf{repeat} until stopping criteria 
		\STATE Localize the next spike:
		$$\tau_{j+1} \in \argmax_{\tau\in\left[0,1\right)} \left| \left\langle \ba(\tau ), \mathcal{A}(\mathcal{T}_{j})\bm{c}_{j} - \bm{z} \right \rangle \right|; $$
		\STATE Update support: $\mathcal{T}_{j+1} \gets \mathcal{T}_{j} \cup \left\{\tau_{j+1}\right\}$;
		\STATE Refinement: \textbf{repeat} \\
		 \begin{enumerate} 
		 \item Update the amplitudes:  
		 $$\bm{c}_{j+1} \leftarrow \argmin\limits_{\left\Vert \bm{c} \right\Vert_1 \leq \eta} \; \frac{1}{2} \left\| \mathcal{A}({\mathcal{T}}_{j+1}) \bc - \bm{z}\right\|_2^2; $$
		\item Prune support: $\mathcal{T}_{j+1} \gets \text{support}({\bm{c}}_{j+1})$;
		\item Locally improve $\mathcal{T}_{j+1}$ by performing local descent with respect to $\tau$;  
		\end{enumerate}
		\STATE $j \gets j+1$;	 
		\ENSURE $\left(  \mathcal{T}_{j }, \bm{c}_{j} \right)$ and $\bm{x}_j = \mathcal{A}(\mathcal{T}_{j})\bm{c}_{j}$.
	\end{algorithmic}
\end{algorithm}


